Anti-LM Decoding for Zero-shot In-context Machine Translation

Zero-shot In-context learning is the phenomenon where models can perform the task simply given the instructions. However, pre-trained large language models are known to be poorly calibrated for this task. One of the most effective approaches to handling this bias is to adopt a contrastive decoding objective, which accounts for the prior probability of generating the next token by conditioning on some context. This work introduces an Anti-Language Model objective with a decay factor designed to address the weaknesses of In-context Machine Translation. We conduct our experiments across 3 model types and sizes, 3 language directions, and for both greedy decoding and beam search ($B=5$). The proposed method outperforms other state-of-art decoding objectives, with up to $20$ BLEU point improvement from the default objective observed in some settings.

==> tables/fr-pt.tex <==
\begin{table}[!h]
\resizebox{\columnwidth}{!}{
\begin{tabular}{lrrrrr}
\toprule

model    & base & PMI(u) & PMI(x) & ALM(u) & ALM(x)        \\
\midrule
gptn2.7B &     4.7 &   2.2 &   3.0 &       4.8 &       4.7 (+0.0) \\
xglm2.9B &    18.7 &  21.0 &  20.5 &      21.5 &      21.0 (+2.3) \\
xglm7.5B &    21.3 &  26.2 &  24.9 &      26.8 &      26.7 (+5.4) \\
bloom3b  &    24.8 &  25.9 &  25.5 &      27.1 &      27.4 (+2.6) \\
bloom7b1 &    29.0 &  28.8 &  29.0 &      29.1 &      28.7 \textcolor{red}{(-0.3)} \\
\bottomrule
\end{tabular}}
\caption{BLEU Scores for translating from French to Portuguese (fr-pt) under greedy decoding. In brackets are numeric difference of our proposed method (ALM(x)) from the baseline.`}
\label{tab:fr-pt}
\end{table}
